V2N Service Scaling with Deep Reinforcement Learning

The fifth generation (5G) of wireless networks is set out to meet the stringent requirements of vehicular use cases. Edge computing resources can aid in this direction by moving processing closer to end-users, reducing latency. However, given the stochastic nature of traffic loads and availability of physical resources, appropriate auto-scaling mechanisms need to be employed to support cost-efficient and performant services. To this end, we employ Deep Reinforcement Learning (DRL) for vertical scaling in Edge computing to support vehicular-to-network communications. We address the problem using Deep Deterministic Policy Gradient (DDPG). As DDPG is a model-free off-policy algorithm for learning continuous actions, we introduce a discretization approach to support discrete scaling actions. Thus we address scalability problems inherent to high-dimensional discrete action spaces. Employing a real-world vehicular trace data set, we show that DDPG outperforms existing solutions, reducing (at minimum) the average number of active CPUs by 23% while increasing the long-term reward by 24%.

==> soa.tex <==
\section{Related Work}
\label{sec:soa}
%action space is mostly -1, 0, +1
Effective scaling of resources is vital in several application domains. %with meeting service level agreements as a main objective. 
The utility of auto-scaling resources using ML methods has been investigated not only in the context of network slicing, but also for cloud resources.
% just rephrasing to make shorter Willemijn
% your prior content was good already ;)
% there's a nice related work here, I like it
% I'm just gonna short, as we lack of space
Authors in \cite{verma2021auto} provide a classification
of auto-scaling techniques, namely,
schedule-based or rule-based (pro-active or
reactive). Authors identify that 
threshold-based policies, queuing theory, control theory, time-series
analysis,
and reinforcement learning
are candidate solutions for rule-based
auto-scaling.
% Verma et al. classify auto-scaling techniques as either rule-based or schedule-based, of which rule-based can be either reactive or pro-active. RL based auto-scaling solutions are a combination of pro-active and reactive. The authors mention RL, threshold-based policies, queuing theory, control theory, and time-series analysis as the categories of rule-based auto-scaling \cite{verma2021auto}.
%%%% NOT INSIGHTFUL 
% Gari et al. show that in a variety of works, RL shows tremendous potential in solving decision-making problems in certain complex environments with a certain level of uncertainty \cite{gari2021reinforcement}.
Other works e.g.,~\cite{li2018deep,li2020lstm} %,hua2019gan}
show that RL is a strong candidate to assess
resource management in network slices.
Specifically, variations of
policy gradient methods as
actor-critic networks that utilise the
advantage function~\cite{yan2019intelligent,chen2019learning},
% function~\cite{yan2019intelligent,grondman2012survey,chen2019learning},
have been shown to be successful in 5G radio access slicing.
Furthermore, auto-scaling of virtualized network functions with other ML strategies have been shown to have be successful \cite{subramanya2019machine,rahman2018auto}. However none of them investigates the flexible scaling decisions that can support traffic surges. The explored action space is often limited, such as scaling up/down the number of CPU by one instead of going for an arbitrary number, to avoid the dimension explosion problems with discrete action space.

%% GOOF IF SPACE, mentioned above
% Among the RL algorithms that are used today by researchers, policy gradient methods like actor-critic algorithms are commonly used \cite{grondman2012survey}. Specifically A2C has been shown by Zheyi et al. to be able to handle dynamic resource allocation in cloud data centers \cite{chen2019learning}. 

%%% good to have if we had space, the
%%% reference is included above
% Previous work by Zhao et al. has shown that an LSTM is able to predict short-term car traffic in cities, showing that a ML model can successfully extract a meaningful pattern from traffic data \cite{zhao2017lstm}.


==> system.tex <==
\section{V2N system description}
\label{sec:system}

 For the V2N system, we focus on a road segment in the coverage area of Radio Unit (RU) as depicted in Fig.~\ref{fig:system}. The RU provides connectivity to smartphone users and CAVs along the road. We assume that every CAV uses V2N-based applications such as remote driving, hazard warning etc., and its traffic is processed in the edge of the network to satisfy latency requirements.  We assume smartphones and CAVs are connected to their respective network slices i.e., \emph{slice~1} supporting smartphones' traffic processed in the cloud; and \emph{slice~2} supporting C-V2N traffic processed at the Edge server. 
 
 
 We focus on the workload 
 $W_t\in\mathbb{R}^+$ that C-V2N
 services introduce in \emph{slice 2}
 over time $t$. The workload $W_t$
 refers to the number of CPUs
 required to process on time the
 $P_v$~packets/sec sent by $V_t$
 vehicles. Knowing
 that a CPU processes on time
 (i.e., satisfying C-V2N latency
 constraints) $P_c$~packets/sec,
 the workload is expressed as
 $W_t=\tfrac{P_vV_t}{P_c}$.
 
 
 The goal is that the system in
 Fig.~\ref{fig:system}~distributes the
 C-V2N workload $W_t$ among the Edge CPUs
 to satisfy latency requirements, i.e.,
 the workload dispatched to each CPU
 should satisfy $W_t\leq 1$.
 Moreover, the system should do an efficient
 (vertical) scaling of the number of CPUs
 $N_t\in\mathbb{N}^+$ that it turns on/off to process the
 C-V2N traffic on time. To achieve an
 efficient scaling, we propose using
 an ML agent (see~Fig.~\ref{fig:system})
 that learns the traffic patterns, and
 anticipates to peaks of demand
 by scaling up the number of CPUs.






%where a
%5G base-station (BS) provides network connectivity to smart-phone users and CAVs within a cityroad. Both traffic flows are isolated into
%two different network slices:
%\emph{slice~1} containing smart-phone's
%packets processed in the cloud; and
%\emph{slice~2} holding the CAVs'
%delay-sensitive C-V2N packets
%that is processed in the Edge.
%In this work we focus on dimensioning
%computational resources for the latter
%slice.

% Incoming C-V2N packets lead to a workload
% of $W_t$ CPUs in the Edge server, i.e.,
% more C-V2N packets require more processing
% power in the Edge server. Therefore, in
% some situations the number
% of CPUs in the Edge server $N_t$
% will not suffice $N_t<W_t$, and
% an agent will have to increase the
% number of CPUs (see Fig.~\ref{fig:system}).





\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{IEEEtran/v2n-scaling-commlet.pdf}
    \caption{Considered C-V2N system.}
      \vspace{-1.5em}
    \label{fig:system}
\end{figure}
%Under such circumstances we turn off CPUs at the Edge server that attends the C-V2N traffic of the dedicated slice.

% In summary, in this paper we focus in
% the dimensioning/scaling of computational
% resources at the Edge to meet the demand
% of C-V2N traffic. The scaling decisions
% are taken considering the maximum workload
% that each CPU can attend on time
% (e.g., below 5~ms~\cite{3GPPV2X2}), and
% the goal is to make an efficient use
% of computational resources.


%But this is not necesarily the best solution, as the 5G cell along the road may receive additional
%C-V2N packets from CAVs that were not expected to be within the road (see~Fig.~\ref{fig:system}).


%%% PRIOR CONTENT
%In other words, the road
% may be more congested than expected due to events
% as traffic jams. In case the road foresees more traffic
% than expected -- hence, more CAVs -- the Edge server
% will have to process an increasing arrival of C-V2N
% packets, and it will require an additional CPU(s)
% to satisfy the new demand. In the example of
% Fig.~\ref{fig:system}, the two unexpected CAVs
% required to scale the Edge server by an additional
% CPU to process the new C-V2N packets.

% Conversely, it could also happen that the road has
% less CAVs than expected, and such situation will
% result in turning off one of the Edge server CPUs,
% as it is no longer required to process the small
% amount of C-V2N packets. Whether the Edge server
% scales up or down the number of CPUs, the goal
% is to process the C-V2N traffic on time, e.g.,
% in less than 5~ms.
% As a result, we formulate
% the associated scaling problem in \S\ref{sec:problem}.





